Can Reinforcement Learning Find Stackelberg-Nash Equilibria in General-Sum Markov Games with Myopic Followers?

We study multi-player general-sum Markov games with one of the players designated as the leader and the other players regarded as followers. In particular, we focus on the class of games where the followers are myopic, i.e., they aim to maximize their instantaneous rewards. For such a game, our goal is to find a Stackelberg-Nash equilibrium (SNE), which is a policy pair $(\pi^*, \nu^*)$ such that (i) $\pi^*$ is the optimal policy for the leader when the followers always play their best response, and (ii) $\nu^*$ is the best response policy of the followers, which is a Nash equilibrium of the followers' game induced by $\pi^*$. We develop sample-efficient reinforcement learning (RL) algorithms for solving for an SNE in both online and offline settings. Our algorithms are optimistic and pessimistic variants of least-squares value iteration, and they are readily able to incorporate function approximation tools in the setting of large state spaces. Furthermore, for the case with linear function approximation, we prove that our algorithms achieve sublinear regret and suboptimality under online and offline setups respectively. To the best of our knowledge, we establish the first provably efficient RL algorithms for solving for SNEs in general-sum Markov games with myopic followers.

==> regret.tex <==
\section{Regret Analysis}
In this section, we establish an upper bound of regret of Model-Based OPPO  (Algorithm \ref{alg:1}) in the following theorem. 

Our analysis relies on the following two assumptions.


\begin{assumption} \label{assumption:feature}
	There exists positive parameters $C_M$, $C_\eta$, $C_\psi$ and $C_\psi'$ such that \\
	$
	\begin{array}{l}\text { 1. }\left\|M^{*}\right\|_{F}^{2} \leq C_{M} \cdot d \\ \text { 2. } \forall(s, a) \in \mathcal{S} \times \mathcal{A}: \quad\|\eta(s, a)\|_{2}^{2} \leq C_{\eta} d \\ \text { 3. } \forall v \in \mathbb{R}^{S}: \quad\left\|\Psi^{\top} v\right\|_{\infty} \leq C_{\psi}\|v\|_{\infty}, \quad \text { and } \quad\left\|\Psi K_{\psi}^{-1}\right\|_{2, \infty} \leq C_{\psi}^{\prime}.\end{array} 
	$
\end{assumption}
See \cite{yang2019reinforcement}.


\begin{assumption} \label{assumption:tv}
	There exists a constant $B_{TV} > 0$ such that $\sum_{k=1}^K \| \theta_h^{k-1} - \theta_h^k \|_2 \le B_{TV}$ for any $h \in [H]$.
\end{assumption}
See \cite{besbes2014stochastic, russac2019weighted}.









\begin{theorem} \label{thm:regret}
	Suppose Assumptions \ref{assumption:linear:reward}, \ref{assumption:transition}, \ref{assumption:feature}, and \ref{assumption:tv} hold. Let $\alpha = \sqrt{2 \log | \cA | /H^2K}$ and $\beta_k' \geq c (C_M + {C_\psi'}^2) \cdot \log (2kHC_\eta/p)\cdot d$ for some sufficiently large constant $c>0$. Assuming that $\log | \cA | = \cO\bigl(d^3 \cdot  \log(T)^2 \bigr)$,  we have 
	\$
	Regret(T) \le \cO(dT) + \cO\bigl(\log(T) \cdot \sqrt{d^3H^3T}\bigr)
	 \$ 
	with probability at least $1-p$.
\end{theorem}
\begin{proof}
	See Section \ref{sec:sketch} for a proof sketch and Appendix \ref{appendix:proof:regret} for a detailed proof.
\end{proof}











==> sketch.tex <==
\iffalse
\section{Proofs of the Main Results}
In this section, we provide the proof of Theorem \ref{thm:offline}. 

\subsection{Proof of Theorem \ref{thm:offline}} \label{sec:pf:thm:offline}
\begin{proof}
For the simplicity of discussion, we define the model prediction errors as
\# \label{eq:def:td:error}
&\delta_{\star, h}^k = r_{\star, h}^k + \PP_h V_{\star, h+1}^k - Q_{\star, h}^k, \quad \star \in \{l, f\}.
%&\delta_{f, h}^k = r_{f, h}^k + \PP_h V_{f, h+1}^k - Q_{f, h}^k.
\#
%By the definition of $Q_{\star, h}^k$ in \eqref{eq:evaluation} and the leader-controller assumption (Assumption \ref{assumption:linear}), we know that $\delta_{\star, h}$ is a function from $\cS \times \cA$ to $\RR$.
Moreover, we define $\zeta_{\star, k, h}^1$ and $\zeta_{\star, k, h}^2$ as 
{\small
\begin{equation}
\begin{aligned} \label{eq:def:martingale}
&\zeta_{\star, k, h}^1 = [V_{\star, h}^k(x_h^k) - V_{\star, h}^{\pi^k, \nu^k}(x_h^k)] - [Q_{\star, h}^k(x_h^k, a_h^k, b_h^k) - Q_{\star, h}^{\pi^k, \nu^k}(x_h^k, a_h^k, b_h^k)], \\
&\zeta_{\star, k, h}^2 = [(\PP_h V_{\star, h+1}^k)(x_h^k, a_h^k, b_h^k) - (\PP_h V_{\star, h+1}^{\pi^k, \nu^k})(x_h^k, a_h^k, b_h^k)] - [V_{\star, h+1}^k(x_{h+1}^k) - V_{\star, h+1}^{\pi^k, \nu^k}(x_{h+1}^k)],
\end{aligned}
\end{equation}
}
where $\star \in \{l, f\}$. Recall that $(\pi^k, \nu^k)$ are the policies executed by the player and the follower in the $k$-th episode, which generate a trajectory $\{x_h^k, a_h^k, b_h^k\}_{h \in [H]}$. Thus, we know that $\zeta_{\star, k, h}^1$ and $\zeta_{\star, k, h}^2$ characterize the randomness of choosing actions $a_h^k \sim \pi_h^k(\cdot \,|\, x_h^k)$ and $b_h^k \sim \nu_h^k (\cdot \,|\, x_h^k)$ and the randomness of drawing the next state $x_{h + 1}^k \sim \cP_h(\cdot \,|\, x_h^k, a_h^k, b_h^k)$, respectively.

To establish an upper bound for the regret defined in \eqref{eq:def:regret}, we introduce the following lemma, which decomposes the regret into three parts using the notations defined above. 


\begin{lemma}[Regret Decomposition]  \label{lemma:decomposition1}
    The regret defined \eqref{eq:def:regret} can be decomposed as
    \$
    %\text{Regret}_l(K) &= \sum_{k = 1}^K [V_{l, 1}^{\pi^*, \nu^*}(x_1^k) - V_{l, 1}^{\pi^k, \nu^k}(x_1^k)] \\
    \text{Regret}_l(K) & =   \underbrace{\sum_{k = 1}^K\sum_{h=1}^H\EE_{\pi^*, \nu^*}[\la Q_{l,h}^k(x_h^k, \cdot, \cdot), \pi_h^*(\cdot \,|\, x_h^k) \times \nu_h^*(\cdot \,|\, x_h^k) -  \pi_h^k(\cdot \,|\, x_h^k) \times \nu_h^k(\cdot \,|\, x_h^k) \ra]}_{{(l.1):} \text{ Computational Error}} \\
    & \quad + \underbrace{\sum_{k = 1}^K\sum_{h=1}^H \bigl(\EE_{\pi^*, \nu^*}[\delta_{l, h}^k(x_h, a_h, b_h)] - \delta_{l, h}^k(x_h^k, a_h^k, b_h^k) \bigr)}_{(l.2): \text{ Statistical Error}} + \underbrace{\sum_{k = 1}^K\sum_{h = 1}^H (\zeta_{l, k, h}^1 + \zeta_{l, k, h}^2)}_{(l.3): \text{ Randomness}}, \\
    %\$
    %\$
    %\text{Regret}_f(K) &= \sum_{k = 1}^k [V_{f, 1}^{\pi^k, \nu^*(\pi^k)}(x_1^k) - V_{f, 1}^{\pi^k, \nu^k}(x_1^k) ] \\
    \text{Regret}_f(K)& = \underbrace{\sum_{k = 1}^K\sum_{h=1}^H \EE_{\pi^k, \nu^*(\pi^k)}[\la Q_{f,h}^k(x_h^k, \cdot, \cdot), \pi_h^k(\cdot \,|\, x_h^k) \times (\nu_h^*(\pi^k)(\cdot \,|\, x_h^k) -  \nu_h^k(\cdot \,|\, x_h^k)) \ra]}_{(f.1): \text{ Computational Error}} \\
    & \quad + \underbrace{\sum_{k = 1}^K\sum_{h=1}^H \bigl(\EE_{\pi^k, \nu^*(\pi^k)}[\delta_{f, h}^k(x_h, a_h, b_h)] - \delta_{f, h}^k(x_h^k, a_h^k, b_h^k) \bigr)}_{(f.2): \text{ Statistical Error}} + \underbrace{\sum_{k = 1}^K\sum_{h = 1}^H (\zeta_{f, k, h}^1 + \zeta_{f, k, h}^2)}_{(f.3): \text{ Randomness}}.
    \$ 
\end{lemma}

\begin{proof}
    See Appendix \ref{appendix:pf:decomposition1} for a detailed proof.
\end{proof}

\begin{remark}
    %can be viewed as the extension of previous results for MDPs 
    Similar regret decomposition results also appear in the single-agent RL literature \citep{cai2020provably,efroni2020optimistic}, and they can be regarded as the special case of Lemma \ref{lemma:decomposition1}.
    Moreover, our regret decomposition lemma is independent of the leader-controller linear setting in Assumption \ref{assumption:linear}, and thus, can be applied to more general settings. 
\end{remark}

Lemma \ref{lemma:decomposition1} states that the regret has three sources: 
(i) computational error, which represents the convergence of the algorithm with the known model, (ii) statistical error, that is, the error caused by the inaccurate estimation of the model, and (iii) randomness, as aforementioned, which comes from executing random policies and interaction with random environment. 

Returning to the main proof, we only need to characterize these three types of errors, respectively. We first characterize the computational error by the following lemma.

\begin{lemma}[Optimization Error] \label{lemma:myopic}
    It holds that 
    \$
    &\sum_{k = 1}^K\sum_{h=1}^H\EE_{\pi^*, \nu^*}[\la Q_{l,h}^k(x_h^k, \cdot, \cdot), \pi_h^*(\cdot \,|\, x_h^k) \times \nu_h^*(\cdot \,|\, x_h^k) -  \pi_h^k(\cdot \,|\, x_h^k) \times \nu_h^k(\cdot \,|\, x_h^k) \ra] \le 0, \\
    & \sum_{k = 1}^K\sum_{h=1}^H \EE_{\pi^k, \nu^*(\pi^k)}\big[\big\la Q_{f,h}^k(x_h^k, \cdot, \cdot), \pi_h^k(\cdot \,|\, x_h^k) \times \bigl(\nu_h^*(\pi^k)(\cdot \,|\, x_h^k) -  \nu_h^k(\cdot \,|\, x_h^k)\bigr) \big\ra\big] \le 0 .
    \$
\end{lemma}

\begin{proof}
    See Appendix \ref{appendix:pf:myopic} for a detailed proof.
\end{proof}

%For the statistical error, $\EE_{\pi^*, \nu^*}[\delta_{l, h}^k(x_h, a_h, b_h)]$ and $\EE_{\pi^*, \nu^*(\pi^k)}[\delta_{f, h}^k(x_h, a_h, b_h)]$ is difficult to estimate since the lack of trajectories induced by $(\pi^*, \nu^*)$ and $(\pi^*, \nu^*(\pi^k))$. However, thanks to the bonus functions defined in \eqref{eq:evaluation}, we can

%Lemma \ref{lemma:myopic} states that Terms $(l.1)$ and $(f.1)$ (optimization errors) are non-positive. Together with Lemma \ref{lemma:decomposition1}, we only need to derive an upper bound for the statistical errors and randomness.

Then, we establish an upper bound for the statistical error. 
Due to the uncertainty that arises from only observing limited data, the model prediction errors can be possibly large for the state-action pairs $(x, a, b)$ that are less visited or even unseen. Fortunately, however, we have the following lemma which characterizes the model prediction errors defined in \eqref{eq:def:td:error}. 
%Recall that the bonus functions $\Gamma_{\star, h}^k, \star \in \{l, f\}$ are defined in \eqref{eq:evaluation}.
\begin{lemma}[Optimism] \label{lemma:ucb}
    It holds with probability at least $1 - p/2$ that 
    \$
    -2\min\{H, \Gamma_{\star, h}^k(x, a)\} \le \delta_{\star, h}^k(x, a, b) \le 0 %\quad -2\Gamma_h^k(x, a, b) \le \delta_{l, h}^k(x, a, b) \le 0.
    \$
    for any $(k, h, x, a, b) \in [K] \times [H] \times \cS \times \cA \times \cA$ and $\star \in \{l, f\}$. 
\end{lemma}

\begin{proof}
    See Appendix \ref{appendix:pf:ucb} for a detailed proof.
\end{proof}

Lemma \ref{lemma:ucb} states that $\delta_{\star, h}^k(x, a, b) \le 0$ for any $(x, a, b) \in \cS \times \cA \times \cA$ and $\star \in \{l, f\}$. Combining the definition of model prediction error in \eqref{eq:def:td:error}, we obtain  
\$
Q_{\star, h}^k(x, a, b) \ge r_{\star, h}(x, a, b) + (\PP_hV_{\star, h+1}^k)(x, a, b),
\$
which further implies that the estimated Q-function $Q_{\star, h}^k$ is “optimistic in the face of uncertainty”. Moreover, Lemma \ref{lemma:ucb} implies that $- \delta_{\star, h}^k(x, a, b) \le 2\min\{H+1, \Gamma_{\star, h}^k(x, a)\}$. Thus we only need to establish an upper bound for $2\sum_{k = 1}^K\sum_{h = 1}^H \{H + 1, \Gamma_{\star, h}^k (x_h^k, a_h^k)\}$, which is the total price paid for the optimism. As shown in the following lemma, we can derive an upper bound for this term by the elliptical potential lemma \citep{abbasi2011improved}. 
\begin{lemma} \label{lemma:elliptical}
    For the bonus function $\Gamma_{\star, h}^k$ defined in \eqref{eq:evaluation}, it holds for any $\star \in \{l, f\}$ that
    \$
    2\sum_{k = 1}^K\sum_{h = 1}^H \min\{H, \Gamma_{\star, h}^k (x_h^k, a_h^k)\} \le \cO(\sqrt{d^2H^3T \iota^2}).
    \$
    Here $p \in (0, 1)$ and $\iota = \log(dTH/p)$ are defined in Theorem \ref{thm:offline}.
\end{lemma} 

\begin{proof}
    See Appendix \ref{appendix:pf:elliptical} for a detailed proof.
\end{proof}

It remains to analyze the randomness, which is the purpose of the following lemma.

\begin{lemma} \label{lemma:martingale}
    For the $\zeta_{\star, k, h}^1$ and $\zeta_{\star, k, h}^2$ defined in \eqref{eq:def:martingale} and any $p \in (0, 1)$,  it holds with probability at least $1 - p/2$ that 
    \$
    \sum_{k = 1}^K\sum_{h = 1}^H (\zeta_{\star, k, h}^1 + \zeta_{\star, k, h}^2) \le \sqrt{16KH^3 \cdot \log(4/p)}.
    \$
    Here $\star \in \{l, f\}$.
\end{lemma}

\begin{proof}
    See Appendix \ref{sec:pf:martingale} for a detailed proof.
\end{proof}

Therefore, we conclude the proof of Theorem \ref{thm:offline}.

\end{proof} 

\subsection{Proof of Theorem \ref{thm:multi:follower}}

\fi
